Matting Anything

In this paper, we propose the Matting Anything Model (MAM), an efficient and versatile framework for estimating the alpha matte of any instance in an image with flexible and interactive visual or linguistic user prompt guidance. MAM offers several significant advantages over previous specialized image matting networks: (i) MAM is capable of dealing with various types of image matting, including semantic, instance, and referring image matting with only a single model; (ii) MAM leverages the feature maps from the Segment Anything Model (SAM) and adopts a lightweight Mask-to-Matte (M2M) module to predict the alpha matte through iterative refinement, which has only 2.7 million trainable parameters. (iii) By incorporating SAM, MAM simplifies the user intervention required for the interactive use of image matting from the trimap to the box, point, or text prompt. We evaluate the performance of MAM on various image matting benchmarks, and the experimental results demonstrate that MAM achieves comparable performance to the state-of-the-art specialized image matting models under different metrics on each benchmark. Overall, MAM shows superior generalization ability and can effectively handle various image matting tasks with fewer parameters, making it a practical solution for unified image matting. Our code and models are open-sourced at https://github.com/SHI-Labs/Matting-Anything.

==> tables/ablation.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{c|c|cc|cc}
&Model &\multicolumn{2}{c}{Synthetic Subset} &\multicolumn{2}{c}{Natural Subset}\\
Method  & Size  &IMQ$_{mad}$$\uparrow$ &IMQ$_{mse}$$\uparrow$ &IMQ$_{mad}$$\uparrow$ &IMQ$_{mse}$$\uparrow$  \\ \hline
%SAM &93.7 M &8.71 &11.06 &11.70 &14.11  \\
SAM~\cite{kirillov2023segment} &93.7 M &31.31 &39.67 &50.47 &61.66  \\
+ Mask-Select &93.7 M &49.69 &61.44 &61.15 &74.01  \\  \hline
MAM Baseline & + 1.0 M &41.72 &58.34  &52.82 &71.82  \\
+ Multi-Scale Prediction & + 2.7 M &44.98 &61.23 &60.11 &74.74  \\
+ Iterative Refinement & + 2.7 M  &49.25 &63.27 &65.44 &78.93\\
+ Multi-Dataset Training & + 2.7 M &53.66 &68.74 &68.37 &81.56 \\
\hline
\end{tabular}
\caption{Ablation study of MAM on the HIM2K benchmark. The MAM Baseline is built upon the SAM model with the box prompt. The other strategies are gradually added to the MAM Baseline and end up with 2.7 M extra trainable parameters.}
\label{tab:ablation}
\vspace{-2mm}
\end{table*}

==> tables/am2k.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{c|c|cccccc}
Method &Size &SAD$_{all}$$\downarrow$ &MSE$_{all}$$\downarrow$  &MAD$_{all}$$\downarrow$ &Grad$_{all}$$\downarrow$ &Conn$_{all}$$\downarrow$ &SAD$_{tri}$$\downarrow$ \\ \hline
SHM   &79.3 M &17.81 &6.8 &10.2 &12.54 &17.02 &10.26 \\
LF  &37.91 M &36.12  &11.6 &21.0 &21.06 &33.62 &19.68  \\ 
HATT & 107.0 M &28.01 &5.5 & 16.1 &18.29 &17.76   &13.36 \\ 
SHMC  & 78.23 M &61.50 &27.0 &35.6 &37.00 &60.94 &35.23  \\ 
GFM-R$^*$ & 55.3 M &10.89 &2.9 &6.4 &10.00 &9.99 &9.15  \\
GFM-D$^*$ & 47.0 M &10.26 &2.9 &5.9 &8.82 & 9.57 &8.24  \\
\hline
SAM & 93.7 M &25.00 & 10.8 &14.8 &60.01 &8.40 &20.72  \\
MAM & 2.7 M &17.34 &6.4 &10.3&18.47 &8.04 &13.13 \\
\hline
\end{tabular}
\vspace{1.5mm}
\caption{Results on the semantic image matting benchmark AM2K. Metrics with \textit{all} and \textit{tri} as subscript indicates the evaluation of the whole image and the transition area, separately. $\downarrow$ means lower values indicate better performance for the metric.$*$ indicates the model is specifically designed for the AM2K benchmark. } 
\label{tab:am2k}
\end{table*}

==> tables/others.tex <==
%%% HIM2K
%% only natural IMQ_mse IMQ_mad
%% 100k 
%% MAM 2010 mask-guide 67.75 80.53
%% MAM 2010 mask-guide twoside 65.94 78.79
%% MAM 3015 mask-guide 66.22 79.28
%% MAM 3015 mask-guide twoside 63.75 76.88
%% MAM 2010 os8-guide 14.60 25.37 
%% MAM 2010 box-guide 44.10 57.66
%% 20k 
%% *** MAM 2010 mask-guide oneside 68.78 81.67
%% MAM 2010 mask-guide twoside 67.69 80.73


%%% RWP636
%% 100k 
%% MAM 2010 mask-guide 54.38 64.34
%% MAM 2010 box-guide  52.35 73.95

%% 20k 
%% *** MAM 2010 box-guide oneside  54.40 76.45
%%  MAM 2010 box-guide twoside 54.41 76.31 
%%  MAM 3015 box-guide twoside 54.41 76.51 

%%%% PPM100
%% 20k
%MAM mask-guide 8.4 11.7 
% *** MAM box-guide  4.6 9.9
%MAM box-guide twoside 4.7 9.10

%%%% AM2k
%% 20k
%MAM mask-guide 19.1 7.4 11.3 22.47 14.69
%***MAM box-guide  17.30 3.5 10.1  10.65 15.67 

%%%% PM10k
%MAM mask-guide 45.xx 
%***MAM box-guide 25.82 9.2 15.4 14.22 23.99

%%%% PM10k
%MAM mask-guide 45.xx 
%***MAM box-guide 25.82 9.2 15.4 14.22 23.99

%%%% RW100
%MAM point mask-guide 207.89 119.8 121.4
%***MAM point box-guide 168.82 89.6 97.7

%*** MAM box mask-guide 29.24 15.1 16.6

% *** MAM text mask-guide 120.10 65.9 67.5
% MAM text box-guide 122.73 64.4 69.1 


%%%% VideoMatte240k
% MAM box-guide 13.75 7.23 2.16 0.57



==> tables/p10k.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{table*}[tb]
\centering
%\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|cccccc}
%&Model &\multicolumn{4}{c}{Metric $\downarrow$} \\
Method &Size &SAD$_{all}$$\downarrow$ &MSE$_{all}$$\downarrow$  &MAD$_{all}$$\downarrow$ &Grad$_{all}$$\downarrow$ &Conn$_{all}$$\downarrow$ &SAD$_{tri}$$\downarrow$ \\ \hline
SHM   &79.3 M &16.64 &6.9 &9.7 &14.54 &16.13  &8.53  \\
LF  &37.91 M &37.51  &15.2 &15.2 &21.82 &36.92 &16.36  \\ 
HATT & 107.0 M &22.66 &3.8 & 13.1 &15.16 &11.95  &9.32 \\ 
SHMC  & 78.23 M &57.85 &29.1 &34.0 &37.28 &57.86 &23.04  \\ 
GFM-D$^*$ & 47.0 M &11.89 &4.1 &6.9 &12.90 & 11.24 &7.80  \\
GFM-R$^*$ & 55.3 M &11.52 &3.8 &6.7 &13.07 &10.83 &8.00  \\

\hline
SAM & 93.7 M &44.11 & 28.8 &25.7 &24.56 &8.62 &31.96  \\
MAM & 2.7 M &26.66 &9.4 &15.8&14.09 &13.08 &24.00 \\
%MAM no mask & 2.7 M &17.86 &6.7 &10.6 &18.84 &8.04 &13.71 \\
\hline
\end{tabular}
\vspace{1.5mm}
\caption{Results on the semantic image matting benchmark PM-10K. Metrics with \textit{all} and \textit{tri} as subscript indicates the evaluation of the whole image and the transition area, separately. $\downarrow$ means lower values indicate better performance for the metric. $*$ indicates the model is specifically designed for the PM-10K benchmark.} 
\vspace{-2mm}
\label{tab:p10k}
\end{table*}

==> tables/rim.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{c|c|ccc}
Method &Prompt &SAD$_{all}$$\downarrow$ &MSE$_{all}$$\downarrow$ &MAD$_{all}$$\downarrow$\\ \hline
MDETR-R101~\cite{kamath2021mdetr} &text  &131.58 &67.5 &75.1 \\
CLIPSeg-ViT-B/16~\cite{luddecke2022image} &text &211.86 &117.8 &122.2 \\
\gr{CLIPMat-ViT-B/16-Refiner}~\cite{li2023referring} &\gr{text} &\gr{107.81} &\gr{59.5} &\gr{62.0} \\
\gr{CLIPMat-ViT-L/16-Refiner}~\cite{li2023referring} &\gr{text} &\gr{85.83} &\gr{47.4} &\gr{49.5} \\
\hline
SAM~\cite{kirillov2023segment} &text &122.76 &67.9 &69.0  \\ 
MAM &text &120.10 &65.9 &67.5 \\ \hline
SAM~\cite{kirillov2023segment} &point &214.19 &123.8 &124.9  \\ 
MAM &point &168.82 &89.6 &97.7\\ \hline
SAM~\cite{kirillov2023segment} &box &33.51 & 17.9 &19.0  \\ 
MAM &box &29.24 &15.1 &16.6 \\
\hline
\end{tabular}
\caption{Results on the referring image matting benchmark RefMatte-RW100. The box prompt can reach a significantly better performance than the text prompt for referring image matting.}
\vspace{-2mm}
\label{tab:refer}
\end{table*}

==> tables/videomatte.tex <==
\begin{table}[tb]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccccc}
Method &MAD$_{all}$ $\downarrow$ &MSE$_{all}$ $\downarrow$ &Grad$_{all}$ $\downarrow$ &Conn$_{all}$ $\downarrow$ &dtSSD$_{all}$$\downarrow$\\ \hline
DeepLabV3 &14.47 &9.67 &8.55 &1.69 & 5.18 \\
FBA &8.36 &3.37 &2.09 &0.75 &2.09 \\
BGMv2 &25.19 &19.63 &2.28 &3.26 &2.74 \\
MODNet &9.41 &4.30 &1.89 &0.81 &2.23 \\
RVM$^*$ &6.08 &1.47 &0.88 &0.41 &1.36\\
\hline
SAM &15.73  &10.93 &5.44 &0.88 &4.27 \\ 
MAM &13.75 &7.23 &2.16 &0.57 &4.21 \\ \hline
\end{tabular}}
\caption{Results on the semantic video matting benchmark VideoMatte240K~\cite{lin2021real}. $*$ indicates the model is specifically designed for the VideoMatte240K benchmark.}
%\vspace{-5mm}
\label{tab:videomatte}
\end{table}
